Navigating Resource Conflicts: Co-opetition and Fairness

In today's dynamic and interconnected world, resource constraints pose significant challenges across various domains, ranging from networks, logistics and manufacturing to project management and optimization, etc. Resource-constrained problems (RCPs) represent a class of complex computational problems that require efficient allocation and utilization of limited resources to achieve optimal outcomes. This thesis aims to delve into such problems involving multiple agents, where agents aim to enhance their own payoffs, or a neutral moderator aims to maximise the system revenue while distributing the resources appropriately among all agents. In the former type of problems, agents may seek collaboration to achieve higher individual shares, resulting in a cooperative game with competition, i.e., co-opetition. Cooperative and non-cooperative game theory tools are utilized to analyze such games. On the other hand, for the latter kind of problems, we use tools from optimization and Markov decision processes.

==> References/mybibfile.tex <==
@article{hallikainen1986dielectric,
	title={Dielectric properties of snow in the 3 to 37 {GHz} range},
	author={Hallikainen, Martti T and Ulaby, Fawwazt T and Abdelrazik, Mohamed},
	journal={Antennas and Propagation, IEEE Transactions on},
	volume={34},
	number={11},
	pages={1329--1340},
	year={1986},
	publisher={IEEE}
}@article{karsten,
  title={Resource pooling and cost allocation among independent service providers},
  author={Karsten, Frank and Slikker, Marco and Van Houtum, Geert-Jan},
  journal={Operations Research},
  volume={63},
  number={2},
  pages={476--488},
  year={2015},
  publisher={INFORMS}
}

@article{abe2017non,
  title={The non-emptiness of the core of a partition function form game},
  author={Abe, Takaaki and Funaki, Yukihiko},
  journal={International Journal of Game Theory},
  volume={46},
  pages={715--736},
  year={2017},
  publisher={Springer}
}


@artilce{5g,
title = {Understanding mmWave Spectrum for 5G Networks. \url{https://www.5gamericas.org/wp-content/uploads/2020/12/InDesign-Understanding-mmWave-for-5G-Networks.pdf}},
\author={5G Americas},
\journal={Downloadable from \url{https://www.5gamericas.org/wp-content/uploads/2020/12/InDesign-Understanding-mmWave-for-5G-Networks.pdf}}}

@inproceedings{orikumhi2018location,
  title={Location-aware coordinated beam alignment in mmWave communication},
  author={Orikumhi, Igbafe and Kang, Jeongwan and Park, Chansik and Yang, Jinmo and Kim, Sunwoo},
  booktitle={2018 56th Annual Allerton Conference on Communication, Control, and Computing (Allerton)},
  pages={386--390},
  year={2018},
  organization={IEEE}
}



@inproceedings{shokri2015beam,
  title={Beam-searching and transmission scheduling in millimeter wave communications},
  author={Shokri-Ghadikolaei, Hossein and Gkatzikis, Lazaros and Fischione, Carlo},
  booktitle={2015 IEEE international conference on communications (ICC)},
  pages={1292--1297},
  year={2015},
  organization={IEEE}
}

@inproceedings{lee2019beam,
  title={Beam alignment and user scheduling in mmWave networks under mobility},
  author={Lee, Jihyun and Ekici, Eylem},
  booktitle={2019 International Symposium on Modeling and Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOPT)},
  pages={1--8},
  year={2019},
  organization={IEEE}
}
@article{he2022cross,
  title={Cross-Layer Optimization: Joint User Scheduling and Beamforming Design with QoS Support in Joint Transmission Networks},
  author={He, Shiwen and An, Zhenyu and Zhu, Jianyue and Zhang, Min and Huang, Yongming and Zhang, Yaoxue},
  journal={IEEE Transactions on Communications},
  year={2022},
  publisher={IEEE}
}

@article{itc,
  title={AoI-Based Opportunistic-Fair mmWave Schedulers},
  author={Singhal, Shiksha and Kavitha, Veeraruna and Ramanath, Sreenath},
  journal={arXiv preprint arXiv:2211.01667. Accepted at International Teletraffic Conference ITC 34},
  year={2022}
}

@article{3Gmeeting,
title = {The Third Generation Partnership Project Technical Specification Group Radio Access Network meeting \#99					 RP-230327
3 },
journal = {Downloadable from \url{https://portal.3gpp.org/ngppapp/TdocList.aspx?meetingId=39912}},
year = {Rotterdam, Netherlands, March 20th – 23rd, 2023}}

@article{ieee2007ieee,
  title={IEEE Standard for Information technology-Telecommunications and information exchange between systems-Local and metropolitan area networks-Specific requirements Part 11: Wireless LAN Medium Access Control (MAC) and Physical Layer (PHY) Specifications},
  author={IEEE Computer Society LAN/MAN Standards Committee and others},
  journal={IEEE Std 802.11\^{}},
  year={2007}
}

@article{wang2009beam,
  title={Beam codebook based beamforming protocol for multi-Gbps millimeter-wave WPAN systems},
  author={Wang, Junyi and Lan, Zhou and Pyo, Chang-woo and Baykas, Tuncer and Sum, Chin-sean and Rahman, Mohammad Azizur and Gao, Jing and Funada, Ryuhei and Kojima, Fumihide and Harada, Hiroshi and others},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={27},
  number={8},
  pages={1390--1399},
  year={2009},
  publisher={IEEE}
}

@article{li2012efficient,
  title={On the efficient beam-forming training for 60GHz wireless personal area networks},
  author={Li, Bin and Zhou, Zheng and Zou, Weixia and Sun, Xuebin and Du, Guanglong},
  journal={IEEE Transactions on Wireless Communications},
  volume={12},
  number={2},
  pages={504--515},
  year={2012},
  publisher={IEEE}
}

@inproceedings{khalili2020optimal,
  title={On optimal multi-user beam alignment in millimeter wave wireless systems},
  author={Khalili, Abbas and Shahsavari, Shahram and Khojastepour, Mohammad A Amir and Erkip, Elza},
  booktitle={2020 IEEE International Symposium on Information Theory (ISIT)},
  pages={2953--2958},
  year={2020},
  organization={IEEE}
}


@article{info_efficient,
  title={Opportunistic scheduling in cellular systems in the presence of noncooperative mobiles},
  author={Kavitha, Veeraruna and Altman, Eitan and El-Azouzi, Rachid and Sundaresan, Rajesh},
  journal={IEEE Transactions on Information Theory},
  volume={58},
  number={3},
  pages={1757--1773},
  year={2012},
  publisher={IEEE}
}

@inproceedings{patra2015smart,
  title={Smart mm-wave beam steering algorithm for fast link re-establishment under node mobility in 60 GHz indoor WLANs},
  author={Patra, Avishek and Simi{\'c}, Ljiljana and M{\"a}h{\"o}nen, Petri},
  booktitle={Proceedings of the 13th ACM International Symposium on Mobility Management and Wireless Access},
  pages={53--62},
  year={2015}
}

@inproceedings{zhang2016tracking,
  title={Tracking angles of departure and arrival in a mobile millimeter wave channel},
  author={Zhang, Chuang and Guo, Dongning and Fan, Pingyi},
  booktitle={2016 IEEE international conference on communications (ICC)},
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@article{alkhateeb2018deep,
  title={Deep learning coordinated beamforming for highly-mobile millimeter wave systems},
  author={Alkhateeb, Ahmed and Alex, Sam and Varkey, Paul and Li, Ying and Qu, Qi and Tujkovic, Djordje},
  journal={IEEE Access},
  volume={6},
  pages={37328--37348},
  year={2018},
  publisher={IEEE}
}

@inproceedings{zhang2021deep,
  title={Deep learning-based coordinated beamforming for massive MIMO-enabled heterogeneous networks},
  author={Zhang, Yinghui and Zhang, Biao and Wang, Huayu and Zhang, Tiankui and Qian, Yi},
  booktitle={2021 IEEE Global Communications Conference (GLOBECOM)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}


@article{karsten2014,
  title={Domain extensions of the Erlang loss function: Their scalability and its applications to cooperative games},
  author={Karsten, Frank and Slikker, Marco and van Houtum, Geert-Jan},
  journal={Probability in the Engineering and Informational Sciences},
  volume={28},
  number={4},
  pages={473--488},
  year={2014},
  publisher={Cambridge University Press}
}

@article{aumann1961,
  title={The core of a cooperative game without side payments},
  author={Aumann, Robert J},
  journal={Transactions of the American Mathematical Society},
  volume={98},
  number={3},
  pages={539--552},
  year={1961}
}

@book{narahari,
  title={Game theory and mechanism design},
  author={Narahari, Yadati},
  volume={4},
  year={2014},
  publisher={World Scientific}
}

@article{anily2010,
  title={Cooperation in service systems},
  author={Anily, Shoshana and Haviv, Moshe},
  journal={Operations Research},
  volume={58},
  number={3},
  pages={660--673},
  year={2010},
  publisher={INFORMS}
}

@book{anily2011,
  title={Homogeneous of degree one games are balanced with applications to service systems},
  author={Anily, Shoshana and Haviv, Moshe},
  year={2011},
  publisher={Tel Aviv University, Faculty of Management, The Leon Recanati Graduate~…}
}

@article{anily2014,
  title={Subadditive and homogeneous of degree one games are totally balanced},
  author={Anily, Shoshana and Haviv, Moshe},
  journal={Operations Research},
  volume={62},
  number={4},
  pages={788--793},
  year={2014},
  publisher={INFORMS}
}

@article{aumann1974cooperative,
  title={Cooperative games with coalition structures},
  author={Aumann, Robert J and Dreze, Jacques H},
  journal={International Journal of game theory},
  volume={3},
  pages={217--237},
  year={1974},
  publisher={Springer}
}

@article{bloch,
  title={Sequential formation of coalitions in games with externalities and fixed payoff division},
  author={Bloch, Francis},
  journal={Games and economic behavior},
  volume={14},
  number={1},
  pages={90--123},
  year={1996},
  publisher={Elsevier}
}

@article{pessimistic,
  title={Expectation formation rules and the core of partition function games},
  author={Bloch, Francis and Van den Nouweland, Anne},
  journal={Games and Economic Behavior},
  volume={88},
  pages={339--353},
  year={2014},
  publisher={Elsevier}
}

@article{WE,
  title={Wardrop equilibria},
  author={Correa, Jos{\'e} R and Stier-Moses, Nicol{\'a}s E},
  journal={Encyclopedia of Operations Research and Management Science. Wiley},
  year={2011},
  publisher={Citeseer}
}

@article{garcia,
  title={Cooperation in Markovian queueing models},
  author={Garc{\'\i}a-Sanz, Mar{\'\i}a Dolores and Fern{\'a}ndez, Francisco R and Fiestras-Janeiro, M Gloria and Garc{\'\i}a-Jurado, Ignacio and Puerto, Justo},
  journal={European Journal of Operational Research},
  volume={188},
  number={2},
  pages={485--495},
  year={2008},
  publisher={Elsevier}
}

@article{gonzalez,
  title={Optimal sharing of surgical costs in the presence of queues},
  author={Gonz{\'a}lez, Paula and Herrero, Carmen},
  journal={Mathematical Methods of Operations Research},
  volume={59},
  pages={435--446},
  year={2004},
  publisher={Springer}
}

@article{hafalir,
  title={Efficiency in coalition games with externalities},
  author={Hafalir, Isa E},
  journal={Games and Economic Behavior},
  volume={61},
  number={2},
  pages={242--258},
  year={2007},
  publisher={Elsevier}
}

@article{CFGs,
  title={Coalition formation games: A survey},
  author={Hajdukov{\'a}, Jana},
  journal={International Game Theory Review},
  volume={8},
  number={04},
  pages={613--641},
  year={2006},
  publisher={World Scientific}
}

@article{harel,
  title={Sharp bounds and simple approximations for the Erlang delay and loss formulas},
  author={Harel, Arie},
  journal={Management Science},
  volume={34},
  number={8},
  pages={959--972},
  year={1988},
  publisher={INFORMS}
}

@article{jagerman,
  title={Some properties of the Erlang loss function},
  author={Jagerman, David L},
  journal={Bell System Technical Journal},
  volume={53},
  number={3},
  pages={525--551},
  year={1974},
  publisher={Wiley Online Library}
}

@article{karsten2012,
  title={Inventory pooling games for expensive, low-demand spare parts},
  author={Karsten, Frank and Slikker, Marco and van Houtum, Geert-Jan},
  journal={Naval Research Logistics (NRL)},
  volume={59},
  number={5},
  pages={311--324},
  year={2012},
  publisher={Wiley Online Library}
}

@article{alpha-core,
  title={Non-emptiness of the alpha-core},
  author={Martins-da-Rocha, Victor Filipe and Yannelis, Nicholas C},
  year={2011},
  publisher={Funda{\c{c}}{\~a}o Getulio Vargas. Escola de P{\'o}s-gradua{\c{c}}{\~a}o em Economia}
}

@article{ozen,
  title={On the core of cooperative queueing games},
  author={{\"O}zen, Ula{\c{s}} and Reiman, Martin I and Wang, Qiong},
  journal={Operations Research Letters},
  volume={39},
  number={5},
  pages={385--389},
  year={2011},
  publisher={Elsevier}
}

@article{ray,
  title={A theory of endogenous coalition structures},
  author={Ray, Debraj and Vohra, Rajiv},
  journal={Games and economic behavior},
  volume={26},
  number={2},
  pages={286--336},
  year={1999},
  publisher={Elsevier}
}

@misc{rudin,
  title={Principles of Mathematical Analysis. vol. 3},
  author={Walter, Rudin},
  year={1964},
  publisher={New York, NY, USA: McGraw-Hill}
}

@article{saad_unilateral,
  title={Coalitional games in partition form for joint spectrum sensing and access in cognitive radio networks},
  author={Saad, Walid and Han, Zhu and Zheng, Rong and Hjorungnes, Are and Basar, Tamer and Poor, H Vincent},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={6},
  number={2},
  pages={195--209},
  year={2011},
  publisher={IEEE}
}

@article{saad,
  title={Coalitional game theory for communication networks},
  author={Saad, Walid and Han, Zhu and Debbah, M{\'e}rouane and Hjorungnes, Are and Basar, Tamer},
  journal={Ieee signal processing magazine},
  volume={26},
  number={5},
  pages={77--97},
  year={2009},
  publisher={IEEE}
}

@article{Shiksha_Perf,
title = {Coalition formation resource sharing games in networks},
journal = {Performance Evaluation},
volume = {152},
pages = {102239},
year = {2021},
issn = {0166-5316},
doi = {https://doi.org/10.1016/j.peva.2021.102239},
url = {https://www.sciencedirect.com/science/article/pii/S0166531621000560},
author = {Shiksha Singhal and Veeraruna Kavitha}
}

@inproceedings{CDC,
  title={Coalition formation in constant sum queueing games},
  author={Singhal, Shiksha and Kavitha, Veeraruna and Nair, Jayakrishnan},
  booktitle={2021 60th IEEE Conference on Decision and Control (CDC)},
  pages={3812--3817},
  year={2021},
  organization={IEEE}
}

@article{lucas,
  title={N-person games in partition function form},
  author={Thrall, Robert M and Lucas, William F},
  journal={Naval Research Logistics Quarterly},
  volume={10},
  number={1},
  pages={281--298},
  year={1963},
  publisher={Wiley Online Library}
}

@inproceedings{timmer,
  title={How to share the cost of cooperating queues in a tandem network?},
  author={Timmer, Judith and Scheinhardt, Werner},
  booktitle={2010 22nd International Teletraffic Congress (lTC 22)},
  pages={1--7},
  year={2010},
  organization={IEEE}
}

@article{yi,
  title={Stable coalition structures with externalities},
  author={Yi, Sang-Seung},
  journal={Games and economic behavior},
  volume={20},
  number={2},
  pages={201--237},
  year={1997},
  publisher={Elsevier}
}

@article{yu,
  title={Capacity sharing and cost allocation among independent firms with congestion},
  author={Yu, Yimin and Benjaafar, Saif and Gerchak, Yigal},
  journal={Production and Operations Management},
  volume={24},
  number={8},
  pages={1285--1310},
  year={2015},
  publisher={Wiley Online Library}
}


@inproceedings{koutsopoulos2010auction,
  title={Auction mechanisms for network resource allocation},
  author={Koutsopoulos, Iordanis and Iosifidis, George},
  booktitle={8th International Symposium on Modeling and Optimization in Mobile, Ad Hoc, and Wireless Networks},
  pages={554--563},
  year={2010},
  organization={IEEE}
}

@article{kelly1997charging,
  title={Charging and rate control for elastic traffic},
  author={Kelly, Frank},
  journal={European transactions on Telecommunications},
  volume={8},
  number={1},
  pages={33--37},
  year={1997},
  publisher={Wiley Online Library}
}

@inproceedings{stoica1996proportional,
  title={A proportional share resource allocation algorithm for real-time, time-shared systems},
  author={Stoica, Ion and Abdel-Wahab, Hussein and Jeffay, Kevin and Baruah, Sanjoy K and Gehrke, Johannes E and Plaxton, C Greg},
  booktitle={17th IEEE Real-Time Systems Symposium},
  pages={288--299},
  year={1996},
  organization={IEEE}
}

@article{kelly1998rate,
  title={Rate control for communication networks: shadow prices, proportional fairness and stability},
  author={Kelly, Frank P and Maulloo, Aman K and Tan, David Kim Hong},
  journal={Journal of the Operational Research society},
  volume={49},
  number={3},
  pages={237--252},
  year={1998},
  publisher={Springer}
}

@article{tun2019wireless,
  title={Wireless network slicing: Generalized kelly mechanism-based resource allocation},
  author={Tun, Yan Kyaw and Tran, Nguyen H and Ngo, Duy Trong and Pandey, Shashi Raj and Han, Zhu and Hong, Choong Seon},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={37},
  number={8},
  pages={1794--1807},
  year={2019},
  publisher={IEEE}
}

@article{xu2019robustness,
  title={On the robustness of price-anticipating kelly mechanism},
  author={Xu, Yuedong and Xiao, Zhujun and Ni, Tianyu and Wang, Jessie Hui and Wang, Xin and Altman, Eitan},
  journal={IEEE/ACM Transactions on Networking},
  volume={27},
  number={4},
  pages={1558--1571},
  year={2019},
  publisher={IEEE}
}



@inproceedings{saad2008distributed,
  title={A distributed merge and split algorithm for fair cooperation in wireless networks},
  author={Saad, Walid and Han, Zhu and Debbah, M{\'e}rouane and Hjorungnes, Are},
  booktitle={ICC Workshops-2008 IEEE International Conference on Communications Workshops},
  pages={311--315},
  year={2008},
  organization={IEEE}
}

@article{Nevrekar2015ATO,
  title={A Theory of Coalition Formation in Constant Sum Games},
  author={Nevrekar, Saish},
  year={2015}
}

@article{yi2003endogenous,
  title={Endogenous formation of economic coalitions: a survey of the partition function approach},
  author={Yi, Sang-Seung},
  journal={Endogenous Formation of Economic Coalitions, Edward Elgar, Cheltenham, UK},
  pages={80--127},
  year={2003}
}


@inproceedings{iturralde2011resource,
  title={Resource allocation using Shapley value in LTE networks},
  author={Iturralde, Mauricio and Yahiya, Tara Ali and Wei, Anne and Beylot, Andr{\'e}-Luc},
  booktitle={2011 IEEE 22nd International Symposium on Personal, Indoor and Mobile Radio Communications},
  pages={31--35},
  year={2011},
  organization={IEEE}
}

@article{kim2016asymptotic,
  title={Asymptotic shapley value based resource allocation scheme for IoT services},
  author={Kim, Sungwook},
  journal={Computer Networks},
  volume={100},
  pages={55--63},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{vulimiri2012well,
  title={How well can congestion pricing neutralize denial of service attacks?},
  author={Vulimiri, Ashish and Agha, Gul A and Godfrey, Philip Brighten and Lakshminarayanan, Karthik},
  booktitle={Proceedings of the 12th ACM SIGMETRICS/PERFORMANCE joint international conference on Measurement and Modeling of Computer Systems},
  pages={137--150},
  year={2012}
}

@inproceedings{reiffers2014game,
  title={Game theory approach for modeling competition over visibility on social networks},
  author={Reiffers-Masson, Alexandre and Hayel, Yezekael and Altman, Eitan},
  booktitle={2014 Sixth International Conference on Communication Systems and Networks (COMSNETS)},
  pages={1--6},
  year={2014},
  organization={IEEE}
}

@article{wei2010game,
  title={A game-theoretic method of fair resource allocation for cloud computing services},
  author={Wei, Guiyi and Vasilakos, Athanasios V and Zheng, Yao and Xiong, Naixue},
  journal={The journal of supercomputing},
  volume={54},
  number={2},
  pages={252--269},
  year={2010},
  publisher={Springer}
}

@inproceedings{cui2011bid,
  title={Bid landscape forecasting in online ad exchange marketplace},
  author={Cui, Ying and Zhang, Ruofei and Li, Wei and Mao, Jianchang},
  booktitle={Proceedings of the 17th ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={265--273},
  year={2011}
}

@article{ma2018complexity,
  title={Complexity study on the Cournot--Bertrand mixed duopoly game model with market share preference},
  author={Ma, Junhai and Sun, Lijian and Hou, Shunqi and Zhan, Xueli},
  journal={Chaos: An Interdisciplinary Journal of Nonlinear Science},
  volume={28},
  number={2},
  pages={023101},
  year={2018},
  publisher={AIP Publishing LLC}
}

@article{johari2004efficiency,
  title={Efficiency loss in a network resource allocation game},
  author={Johari, Ramesh and Tsitsiklis, John N},
  journal={Mathematics of Operations Research},
  volume={29},
  number={3},
  pages={407--435},
  year={2004},
  publisher={INFORMS}
}

@incollection{dhounchak2019participate,
  title={To participate or not in a coalition in adversarial games},
  author={Dhounchak, Ranbir and Kavitha, Veeraruna and Hayel, Yezekael},
  booktitle={Network Games, Control, and Optimization},
  pages={125--144},
  year={2019},
  publisher={Springer}
}

@inproceedings{tejas,
  title={On-demand OFDMA: Control, fairness and non-cooperation},
  author={Kavitha, Veeraruna and Bodas, Tejas and Manjunath, D},
  booktitle={2013 11th International Symposium and Workshops on Modeling and Optimization in Mobile, Ad Hoc and Wireless Networks (WiOpt)},
  pages={224--231},
  year={2013},
  organization={IEEE}
}

@article{mmwave,
  title={User Scheduling and Beam Alignment in mmWave Networks With a Large Number of Mobile Users},
  author={Lee, Jihyun and Ekici, Eylem},
  journal={IEEE Transactions on Wireless Communications},
  volume={20},
  number={10},
  pages={6481--6492},
  year={2021},
  publisher={IEEE}
}

@inproceedings{hassan2018multi,
  title={Multi-user beam-alignment for millimeter-wave networks},
  author={Hassan, Rana A and Michelusi, Nicolo},
  booktitle={2018 Information Theory and Applications Workshop (ITA)},
  pages={1--7},
  year={2018},
  organization={IEEE}
}

@article{kushner,
  title={Convergence of proportional-fair sharing algorithms under general conditions},
  author={Kushner, Harold J and Whiting, Philip A},
  journal={IEEE transactions on wireless communications},
  volume={3},
  number={4},
  pages={1250--1259},
  year={2004},
  publisher={IEEE}
}

@book{Putterman,
  title={Markov decision processes: discrete stochastic dynamic programming},
  author={Puterman, Martin L},
  year={2014},
  publisher={John Wiley \& Sons}
}
@inproceedings{zhao2015resource,
  title={Resource allocation in device-to-device communication underlaid cellular network using SCMA: An opportunistic approach},
  author={Zhao, Kepeng and Shi, Yan and Dai, Yanpeng and Liu, Lei and Liu, Junyu and Sheng, Min and Li, Jiandong},
  booktitle={2015 IEEE/CIC International Conference on Communications in China (ICCC)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@inproceedings{chen2014distributed,
  title={Distributed SIR-aware opportunistic access control for D2D underlaid cellular networks},
  author={Chen, Zheng and Kountouris, Marios},
  booktitle={2014 IEEE Global Communications Conference},
  pages={1540--1545},
  year={2014},
  organization={IEEE}
}

@book{hoel,
  title={Introduction to stochastic processes},
  author={Hoel, Paul G and Port, Sidney C and Stone, Charles J},
  year={1986},
  publisher={Waveland Press}
}

@book{meyn,
  title={Markov chains and stochastic stability},
  author={Meyn, Sean P and Tweedie, Richard L},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{balter,
  title={Performance modeling and design of computer systems: queueing theory in action},
  author={Harchol-Balter, Mor},
  year={2013},
  publisher={Cambridge University Press}
}


@article{AvgtoDiscount,
  title={Average cost optimal stationary policies in infinite state Markov decision processes with unbounded costs},
  author={Sennott, Linn I},
  journal={Operations Research},
  volume={37},
  number={4},
  pages={626--633},
  year={1989},
  publisher={INFORMS}
}

@article{cellular,
  title={Fair scheduling in cellular systems in the presence of noncooperative mobiles},
  author={Kavitha, Veeraruna and Altman, Eitan and El-Azouzi, Rachid and Sundaresan, Rajesh},
  journal={IEEE/ACM Transactions on Networking},
  volume={22},
  number={2},
  pages={580--594},
  year={2013},
  publisher={IEEE}
}

@inproceedings{debayan,
  title={Fairness via priority scheduling},
  author={Kavitha, Veeraruna and Hemachandra, Nandyala and Das, Debayan},
  booktitle={2013 51st Annual Allerton Conference on Communication, Control, and Computing (Allerton)},
  pages={138--145},
  year={2013},
  organization={IEEE}
}

@article{ming,
  title={Millimeter wave communications for future mobile networks},
  author={Xiao, Ming and Mumtaz, Shahid and Huang, Yongming and Dai, Linglong and Li, Yonghui and Matthaiou, Michail and Karagiannidis, George K and Bj{\"o}rnson, Emil and Yang, Kai and Chih-Lin, I and others},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={35},
  number={9},
  pages={1909--1935},
  year={2017},
  publisher={IEEE}
}

@inproceedings{qureshi,
  title={Online Bayesian learning for rate selection in millimeter wave cognitive radio networks},
  author={Qureshi, Muhammad Anjum and Tekin, Cem},
  booktitle={IEEE INFOCOM 2020-IEEE Conference on Computer Communications},
  pages={1449--1458},
  year={2020},
  organization={IEEE}
}

@inproceedings{irmak,
  title={MAMBA: A multi-armed bandit framework for beam tracking in millimeter-wave systems},
  author={Aykin, Irmak and Akgun, Berk and Feng, Mingjie and Krunz, Marwan},
  booktitle={IEEE INFOCOM 2020-IEEE Conference on Computer Communications},
  pages={1469--1478},
  year={2020},
  organization={IEEE}
}

@inproceedings{yuan,
  title={Optimizing freshness of information: On minimum age link scheduling in wireless systems},
  author={He, Qing and Yuan, Di and Ephremides, Anthony},
  booktitle={2016 14th International Symposium on Modeling and Optimization in Mobile, Ad Hoc, and Wireless Networks (WiOpt)},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{kaul,
  title={Real-time status: How often should one update?},
  author={Kaul, Sanjit and Yates, Roy and Gruteser, Marco},
  booktitle={2012 Proceedings IEEE INFOCOM},
  pages={2731--2735},
  year={2012},
  organization={IEEE}
}

@inproceedings{kavitha,
  title={Controlling packet drops to improve freshness of information},
  author={Kavitha, Veeraruna and Altman, Eitan},
  booktitle={International Conference on Network Games, Control and Optimization},
  pages={60--77},
  year={2021},
  organization={Springer}
}

@article{LLN,
  title={Laws of Large numbers for non-homogeneous Markov systems},
  author={Vassiliou, P-CG},
  journal={Methodology and Computing in Applied Probability},
  volume={22},
  number={4},
  pages={1631--1658},
  year={2020},
  publisher={Springer}
}

@book{Benveniste,
  title={Adaptive algorithms and stochastic approximations},
  author={Benveniste, Albert and M{\'e}tivier, Michel and Priouret, Pierre},
  volume={22},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{RL,
  title={Reinforcement learning: An introduction},
  author={Sutton, Richard S and Barto, Andrew G},
  year={2018},
  publisher={MIT press}
}

@article{mayur,
  title={Opportunistic schedulers and asymptotic price for fairness},
  author={Kavitha, Veeraruna and Hemachandra, Nandyala and Zambre, Mayur},
  journal={Computer Communications},
  volume={148},
  pages={27--41},
  year={2019},
  publisher={Elsevier}
}

@article{von1947theory,
  title={Theory of games and economic behavior, 2nd rev},
  author={Von Neumann, John and Morgenstern, Oskar},
  year={1947},
  publisher={Princeton university press}
}

@article{aumann1960neumann,
  title={Von Neumann-Morgenstern solutions to cooperative games without side payments},
  author={Aumann, Robert J and Peleg, Bezalel},
  year={1960}
}

@article{hart1983endogenous,
  title={Endogenous formation of coalitions},
  author={Hart, Sergiu and Kurz, Mordecai},
  journal={Econometrica: Journal of the econometric society},
  pages={1047--1064},
  year={1983},
  publisher={JSTOR}
}

@article{shenoy1979coalition,
  title={On coalition formation: a game-theoretical approach},
  author={Shenoy, Prakash P},
  journal={International journal of game theory},
  volume={8},
  number={3},
  pages={133--164},
  year={1979},
  publisher={Springer}
}

@book{myerson1997game,
  title={Game theory: analysis of conflict},
  author={Myerson, Roger B},
  year={1997},
  publisher={Harvard university press}
}

@inproceedings{minarolli2011utility,
  title={Utility-based resource allocation for virtual machines in cloud computing},
  author={Minarolli, Dorian and Freisleben, Bernd},
  booktitle={2011 IEEE symposium on computers and communications (ISCC)},
  pages={410--417},
  year={2011},
  organization={IEEE}
}

@inproceedings{kumar2011resource,
  title={Resource allocation for real-time tasks using cloud computing},
  author={Kumar, Karthik and Feng, Jing and Nimmagadda, Yamini and Lu, Yung-Hsiang},
  booktitle={2011 proceedings of 20th international conference on computer communications and networks (ICCCN)},
  pages={1--7},
  year={2011},
  organization={IEEE}
}

@article{jain1984quantitative,
  title={A quantitative measure of fairness and discrimination},
  author={Jain, Rajendra K and Chiu, Dah-Ming W and Hawe, William R and others},
  journal={Eastern Research Laboratory, Digital Equipment Corporation, Hudson, MA},
  volume={21},
  year={1984}
}

@book{lan2010axiomatic,
  title={An axiomatic theory of fairness in network resource allocation},
  author={Lan, Tian and Kao, David and Chiang, Mung and Sabharwal, Ashutosh},
  year={2010},
  publisher={IEEE}
}

@article{liu2001opportunistic,
  title={Opportunistic transmission scheduling with resource-sharing constraints in wireless networks},
  author={Liu, Xiaojun and Chong, Edwin K. P. and Shroff, Ness B.},
  journal={IEEE Journal on Selected Areas in Communications},
  volume={19},
  number={10},
  pages={2053--2064},
  year={2001},
  publisher={IEEE}
}

@article{asadi2013survey,
  title={A survey on opportunistic scheduling in wireless communications},
  author={Asadi, Arash and Mancuso, Vincenzo},
  journal={IEEE Communications surveys \& tutorials},
  volume={15},
  number={4},
  pages={1671--1688},
  year={2013},
  publisher={IEEE}
}






















 

==> abbreviations.tex <==
\chapter*{List of Abbreviations}
\label{ch:ListOfAbr}
\addcontentsline{toc}{chapter}{\nameref{ch:ListOfAbr}}

\makeatletter
\newcommand{\tocfill}{\cleaders\hbox{}\hfill}
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
\makeatother
\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{abbreviations}{\begin{list}{}{\renewcommand{\makelabel}{\abbrlabel}
                                              \setlength{\itemsep}{0pt}}}{\end{list}}
%\begin{abbreviations}[labelsep=1em,font=\bfseries]
\begin{abbreviations}
\item[AGU] 	Adaptive Generalized Unitary transformation
\item[API] Application Programming Interface
\item[BSC]	Backscattering Coefficient
\item[SAR]  Synthetic Aperture Radar  
\item[CTD]	Coherent Target Decomposition
\end{abbreviations}


==> chap_05_Comparison.tex <==
\chapter{Stability comparison of online auctions and queueing system}
\label{chap_comp}

In this chapter, we compare the  stability results of the two applications covered in  Chapters~\ref{chap_PEVA} and~\ref{chap_OR}. We consider both the notions of stability, i.e., stability against unilateral and coalitional deviations (see U-core and core respectively in Section \ref{sec:pfg_new_sc} of Chapter \ref{chap_CGT}) for this comparison. We also compare the specifications of the tools used for both applications. %Specifically, we compare the properties of the stable partitions  of the two applications that are stable against against unilateral and coalitional deviations (see U-core and core respectively in Section \ref{sec:pfg_new_sc} of Chapter \ref{chap_CGT}). A partition is said to be stable against unilateral deviations if none of the players can unilaterally change their strategy profile and obtain better payoffs. On the other hand, a partition is said to be stable against coalitional deviations  if players cannot do better by jointly deviating from the current strategy. 

Chapter~\ref{chap_PEVA} considers  online auctions, modeled using Kelly's mechanism, which we refer to as KM system. This chapter proposes an extended version of the Shapley value, defined in   sub-section~\ref{sec_sol_concept_pfg} (also discussed in Section \ref{sec:pfg_new_sc}), to study the problem. In contrast, Chapter~\ref{chap_OR} examines the stability of partitions in a lossy queueing system, referred to as LQ system. This chapter employs a `special' proportional payoff vector, as defined in \eqref{Eqn_PSA}.


\textbf{Comparison against unilateral deviations: } By Corollary~\ref{corollary_ALC_NE}, for the KM system, the only stable partition is the partition in which all players are alone (referred to as ALC partition), provided that the players are identical and their count exceeds four. However, as the `disparity' (differences in the influence factors) among agents increases, the number of stable partitions grows (as evidenced by Theorems \ref{Thm_stable_big_asym},\ref{Thm_Sym_to_Asym}, Tables \ref{tab:case1},\ref{tab:case2}, and Figures \ref{MoA_vs_stable}, \ref{MoA_random}). Once the disparity between the agents  surpasses a threshold, all partitions become stable (as stated in Theorems~\ref{Thm_general} and \ref{Thm_general_sym}). Coming to LQ system, all partitions are stable against unilateral deviations --  there exists at least one (and indeed, infinitely many) stable configuration involving the partition and this is true for all partitions (see Appendix \ref{chap_appendix_comp} for proof). 

\begin{lemma}
  For every partition $\P$, there exists at least one  (and indeed, infinitely many) payoff vector ${\bm \phi}$ consistent with $\P$ such that the configuration $(\P,{\bm \phi})$ is stable against unilateral deviations in the LQ system.
  \label{lem_uni_LQ}
\end{lemma}

\textbf{Stability against coalitional deviations: }By Theorem \ref{Thm_CS_None}, none of the partitions in KM system are stable against coalitional deviations, when the players are symmetric or identical and their number is more than four. While by Theorem \ref{Thm_GC_CS} for asymmetric players,  grand coalition is the only stable partition, under certain conditions. %The partitions in KM system based study examines the stability  of the partitions for symmetric (in Theorem \ref{Thm_CS_None}) and asymmetric players (in Theorem \ref{Thm_GC_CS}). Theorem \ref{Thm_CS_None} shows that none of the partitions are stable when the players are symmetric, while for asymmetric players Theorem \ref{Thm_GC_CS} shows that grand coalition is stable, subject to certain conditions. 
However, no partition is stable for the LQ system (see Theorem \ref{thm_impossible}).

The LQ study also examines stability under newly introduced restrictive blocking/stability notions, which demonstrate the stability of duopolies (see Theorems \ref{Thm_two_partition} and \ref{Thm_stable_config_ruleB}). However, as demonstrated in the KM study, none of the partitions except all being alone (i.e., ALC partition) are stable against unilateral deviations, rendering all of them unstable even under these new (restricted) notions. Also, ALC partition is not stable, as it can be blocked by a merger coalition consisting of all players except one. Nonetheless, the grand coalition remains stable under specific conditions for asymmetric players, implying its stability even under the new restricted stability notions.



==> chap_10_Wireless_ITC.tex <==
\chapter{AoI-Based Opportunistic-Fair mmWave Schedulers}
\label{chap_wireless}

\section{Introduction}
  
With the rapid advancement of technology, the data traffic has increased considerably. Applications like, ultra-high-definition (UHD) 3D video, virtual
and augmented realities, internet-of-things (IoT) etc., demand high data rates. High data rates can be achieved either using high   bandwidth  or transmit power. One cannot increase power arbitrarily  due to health guidelines. To increase bandwidth, the current trend is to use  Millimeter Waves (mmWaves) in the spectral range of 24GHz to 40GHz.   

In mmWave communications, the base station (BS) needs to align the beam in the  direction of the end user.  Beam alignment is a challenging task as the location of the users may not be known apriori and further could be varying continuously.  % Base stations need to identify the direction of users as quickly as possible prior to the data transfer.

Opportunistic schedulers (\hspace{-1.4mm}~\cite{tejas,kushner,cellular,debayan}) are widely used in wireless networks to take advantage of a `kind of diversity gain'; the channel conditions are independent across slots and users; in every slot, the BS seeks  channel estimate of each of the users and selects the `best' user for data transmission. The `best' criterion also includes fairness aspects: some far away users have bad channels with high probability and one still needs to allocate a channel to such users to be fair. Generalized $\alpha$-fair opportunistic  schedulers are designed precisely for this purpose: allocate a channel to deprived users when the opportunities are the `best', to an extent depending upon fairness-level defining parameter $\alpha$.


With mmWave transmissions and its desired accurate beam alignment, it is difficult to obtain the channel estimates from all the users.  Most of the papers (e.g., \cite{ming,qureshi,irmak,mmwave}) that we are aware of select one user in each slot and accurately align the beam towards the selected user prior to data transfer.  Towards designing mmWave-opportunistic scheduler, \textit{we propose to maintain sufficiently accurate user position updates of each user at BS (see Fig. \ref{fig:AoI}).}  With accurate position updates, we assume the beam alignment times to be negligible.
The users can instead transmit the alignment directions, if there are privacy concerns. 

\begin{figure}[!h]
%\vspace{-5.5mm}
    \centering
    \includegraphics[trim = {1cm 3cm 0cm 3cm}, clip, scale = 0.6]{Figures/AOI.pdf}
    \caption{Beam alignment for multiple mobile/static users}
    \label{fig:AoI}
    %\vspace{-1mm}
\end{figure}

 The wireless users are often mobile,
the BS needs  regular updates of the positions of all the users. Our idea is to design an appropriate dual scheduler that considers all relevant aspects,  age-of-information (AoI), opportunistic and fair schedules;  to be precise, the scheduler has to assign a user for position-update and another/the same user for data transfer in each time-slot in an optimal manner. 
In contrast to the existing literature on AoI that optimize average or peak AoI (e.g., \cite{yuan,kaul,kavitha}), we directly consider the well-known $\alpha$-fair objective function (e.g., \hspace{-1.4mm}~\cite{kushner,cellular}) which is constructed using time-average utilities of all the users, which in turn are influenced by individual AoI trajectories.  

Our main contributions are: i) using theoretical and some heuristic (conjecture that needs proof) arguments, we show that the above mentioned objective function reduces to an average cost Markov decision process (MDP) problem; ii) using the well-known MDP solution techniques (e.g., \cite{Putterman}), we propose an online algorithm for the dual scheduler; iii) the dual scheduler is parametrized by $\alpha$ and  achieves various levels of fairness depending upon the choice of $\alpha$;  iv) we introduce fairness-concepts in two different ways in non-opportunistic schedulers, currently  studied  in literature for mmWaves (e.g., \cite{mmwave}); and finally v) the opportunistic and non-opportunistic schedulers  are compared using exhaustive Monte-Carlo simulations.  

%A detailed survey of challenges in the deployment of the mmWave mobile communication is discussed in \cite{ming}, including beam alignment problems.  The authors in \cite{qureshi,irmak} proposed a bandit algorithm to learn the optimal beam directions between the base stations and end-users in a stochastic setting. However, these algorithms only align towards one user, while opportunistic schedulers require accurate position-updates of all users. 

 
 
 

    



 

 


\section{Problem Description and Background}
\label{sec_model_Wireless}


We consider a network consisting of a Base Station (BS) and $N$ mobile/stationary users labeled $n \in \{1,2,\cdots,N\}$. 
Since millimeter waves (mmWaves) are being used for transmission, one needs to employ narrow beams and a good link is established only when the BS is well-aligned with the users; towards this, we propose to maintain accurate estimates of various user positions at BS; in other words,  we need a mechanism by which regular position updates of (all) the  users is obtained. 

%We design such a mechanism by using Age of Information (AoI) metric.  

\noindent {\bf User-position Updates:} The time frame is divided into time-slots, and,  exactly one user's position is updated in each slot.  The age of various position-updates  in slot $k$ is represented by   vector $\G_k = (G^1_k, \cdots, G^N_k)$, where $G_k^n = 1$ implies this position is just updated. 
%which contains information about staleness of position updates of each of the $n$ users.
Say user $n$ updates its position in time slot $k$, then the vector $\G_k$ evolves as follows:
\begin{eqnarray}
\sG_{k+1}^n &\hspace{-3mm}=\hspace{-3mm}& 1, \text{ and, } \\
\sG_{k+1}^i &\hspace{-3mm}=\hspace{-3mm}& \min\left\{\sG_{k}^i+1, \ \bar{g}\right\}%\ind_{\left \{ \sG_{k}^i<\bar{g}\right \}} + \bar{g}\ind_{\left \{ \sG_{k}^i\ge\bar{g}\right \}} 
\text{ for all } i \neq n, \nonumber
\end{eqnarray}
where $\bar{g}$ is the age upper bound at which the beam alignment deteriorates to a condition such that the utility obtained by that user during data transfer is close to zero.

\noindent
\textbf{Data Scheduler:} The remaining time in every slot after position update is used for data transmission. 
Here again exactly one user is allocated the data channel. The main idea of the paper is to consider an \textit{opportunistic} and \textit{fair scheduler} for this purpose.  Towards opportunistic scheduler, the BS aligns beams in directions of each of the users to obtain their channel estimates, $\H_k = (\sH_k^1,\cdots,\sH_k^n)$; here $\sH^n_k = \sA_k^n \sU_k^n$ in time-slot $k$ for user $n$, where  factor  $\sA_k^n$ depends on the age $\sG^n_k$ of user $n$ and accounts for the misalignment, while,     $\{\sU^n_{k}\}_{k}$ are i.i.d. (independent and identically distributed)  across time-slots for any user $n$; the distribution need not be the same for all users. For example, $\sU^n_{k}$ for any $n$ can depend on Rician or Rayleigh channel conditions of that user.  
If $\sG^n_k$ is high, there is a possibility of higher error in beam alignment as the user might have  moved significantly; then the factor $\sA_k^n$ takes smaller values with higher probability. 


%Hence, $\H_k$ is a Markov chain over a finite state space.

%Further, our aim is to consider a scheduler, which is fair. 

\noindent
\textbf{Background on $\mathbf{\alpha}$-Fair Schedulers: }
Fairness is a well-studied concept in wireless networks (e.g., \cite{tejas,kushner,cellular,debayan} and the references therein). Some users are far away from BS while others are nearby. The far away users have inferior channel conditions with high probabilities. Thus, any efficient scheduler (one that maximizes total utility derived because of overall data transfer)  will not be fair to such far away users. 
%
Fair schedulers are proposed to cater to the demands of such deprived users.

An opportunistic and fair scheduler allocates the channel to the deprived users, in a controlled manner and when the `opportunities'  are the best; this ensures the total utility of the system is the best possible under the given constraints. %maintaining allocating the channel (sometimes in between) even to the users with `bad' channel states.
%
The well-known generalised $\alpha$-fair schedulers exactly achieve this at various levels of fairness indicated  by $\alpha$, by optimizing a certain parameterised concave function of the average utilities obtained by each of the users, as below,
%In other words, the central scheduler allocates the channel to the users in such a way that the sum utility of the system is maximized while allocating the channel (sometimes in between) even to the users with `bad' channel states.
%
%An $\alpha$-fair scheduler $\beta$ is obtained by maximizing the following function:
\begin{eqnarray}
 \sup_{\bbeta = (\beta^1, \cdots, \beta^N)} \sum_n  \Gamma_\alpha \left ( \rsbU^n(\bbeta) \right ) \text{ with } \rsbU^n(\bbeta):=E[\sH^n \beta^n (\H)]\ ],\hspace{-10mm} \nonumber  \\
 \Gamma_\alpha(\rsbU) := \frac{\rsbU^{1-\alpha} \ind_{ \left \{ \alpha \neq 1 \right \}} }{1-\alpha} + \log(\rsbU) \ind_{\left \{ \alpha =1 \right \}}. 
 \label{Eqn_alpha_fair}
\end{eqnarray}
This criterion was previously considered for i.i.d. channels $\{\H_k\}$, while one can easily extend it to Markov channels (i.e., when $\{\G_k\}$ is Markov). In the following, we consider Markov $\{\G_k\}$,   and, also summarize the solution of the above:
\begin{lemma}
\label{lem_fixed_pt}
{\it Assume $\{ \G_k \}_k$ is  a Markov chain with  at maximum finitely many irreducible classes, each having unique  stationary distribution,  evolving independently of the data scheduler decisions $ \{\bbeta_{k}\}$.   
 Then there exists a unique solution  $(\rsbU_\alpha^1, \cdots, \rsbU_\alpha^N)$ to the following $N$-dimensional fixed point equation:
 

\vspace{-3mm}
{\small \begin{eqnarray}
\label{Eqn_beta_alpha_FP}
\rsbU_\alpha^n = E^d_{\rX_0}[ \sH^n \beta^n_\alpha (\H) ], \     \beta_\alpha^n (\H) :=\Pi_{i \ne n}  \ind  \left \{ \frac{\sH^n}{ \left (\rsbU_\alpha^n \right )^\alpha }     \ge  \frac{\sH^i}{ \left (\rsbU_\alpha^i \right )^\alpha } \right \}\hspace{-1mm} ,\hspace{-1mm}
\end{eqnarray}}where $E^d_{\rX_0}[\cdot]$ is expectation under stationary distribution(s) and when initialized with $\rX_0$.
Further, $\bbeta_\alpha = (\beta_\alpha^1, \cdots, \beta_\alpha^N)$   optimizes the   $\alpha$-fair criterion \eqref{Eqn_alpha_fair} for any  given $\alpha$.}
\end{lemma}
{\bf Proof:} This is a well known result in literature (e.g., \cite{tejas,cellular} for the case when $\{\H_k\}$ are i.i.d.%, {\color{red}but the proof immediately follows for the Markov chain too.

  Given the initial condition $\rX_0$ and SMR policy $d$, let $\pi^d_{\rX_0}$ be the stationary distribution (S.D.),  an appropriate convex combination of the S.D.s of various irreducible classes or the unique one. Then one can view $\G$ as i.i.d. variables with this measure, as the given expectation does not depend upon the correlations between various time slots of the Markov chains. And now the proof proceeds as in \cite{tejas,cellular}.
 \eop

\textit{The hypothesis of the above lemma is   satisfied as the age vector $\G_k$ takes finitely many values.}  
An online algorithm that asymptotically represents $\alpha$-fair scheduler \eqref{Eqn_beta_alpha_FP} uses the average utilities  derived by the users till slot $k$, represented by $\bU_k = (\sbU^1_{k},\cdots,\sbU^N_k)$, and is given by (e.g., \cite{kushner,cellular}):


\vspace{-4mm}
{\small
\begin{eqnarray}
\sbU^n_{k+1} &=& \sbU^n_k + \frac{1}{k+1} \left ( \sH^n_{k+1} \beta^n_{k+1} - \sbU^n_k \right ),  \nonumber \\
\beta^n_{k+1} &=& \Pi_{i \ne n}  \ind { \left \{ \frac{\sH^n_{k+1}}{ \left (\sbU^n_k \right )^\alpha }     \ge  \frac{\sH^i_{k+1}}{ \left (\sbU^i_k \right )^\alpha } \right \}  }.  \label{Eqn_beta_scheduler}
\end{eqnarray}}
In \cite{kushner,cellular}, it is proved that the above algorithm converges weakly to asymptotic utilities \eqref{Eqn_beta_alpha_FP} for i.i.d. channels. 
%
 Observe from \eqref{Eqn_beta_scheduler} that the data scheduler  $\beta_{k+1}$,   depends on the channel estimates $\{\H_{k+1}\}$ as well as the average utilities %accumulated so far 
 $\bU_{k}$.% = (\sbU^1_{k},\cdots,\sbU^N_k)$. 
 
\noindent 
\textbf{Dual Scheduler: }In view of the above, it is appropriate to consider the age-scheduler that depends upon   $\X_k := \left ( \G_k , \bU_k  \right )$.
Thus to summarise,  we have a dual scheduler in each time slot (see Fig. \ref{fig:time slot division}):  (i) firstly age scheduler
  $d(\X_k)$,  chooses a user  whose position is to be updated, and then, (ii) the data scheduler, $\bbeta(\H_{k+1},\bU_k)$, chooses a user for data transfer.   
  \begin{figure}[!h]
%  \vspace{-3mm}
     \centering
     \includegraphics[trim = {2cm 8cm 3cm 2cm}, clip, scale = 0.5]{Figures/Time_slot.pdf}
     \caption{Time slot in proposed mmWave Network}
     \label{fig:time slot division}
 \end{figure}
  We consider Stationary Markov Randomized (SMR) policies for age-scheduler (e.g., \cite{Putterman}), i.e., $d$ depends only upon $\X_k$. \textit{With slight abuse of notations, we denote any SMR policy by $d$ instead of $d^\infty$.}
  Under such policies, $\X_k$ is a Markov chain which captures the evolution of the entire system.
 %
 
 
\section{ 
  Dual Opportunistic Fair Scheduler (DOFS)}
We are interested in solving the following two level optimization problem (if $\bbeta^*$ exists), constructed using average utilities and  $\alpha$-fair objective function defined in \eqref{Eqn_alpha_fair}:
\begin{eqnarray}
\label{Eqn_opt_original}
  \sup_{d \in {\cal D}^1} \sum_{n=1}^N \sbU^n_\infty (\bbeta^*) && \hspace{-10mm}\mbox{ where }
  \bbeta^* \in 
  \arg \max_{ \bbeta} \sum_{n=1}^N  \Gamma_\alpha \left ( \sbU^n_\infty \right )  \mbox{ with }  %\hspace{-20mm}
  \nonumber 
\\
\sbU^n_\infty &:=&
 \limsup_{T \to \infty} \frac{1}{T}\sum_{k=1}^T  
   \sH_k^n \beta_k^n,
\end{eqnarray}
where the  domain ${\cal D}^1$ includes all the SMR policies.

%which depends on the age of position updates, $\G_k$ as well as the average utilities obtained by each of the users, $\bU_k$.

%Consider any SMR policy $d$ and any $\beta (\H)  = \{\beta^n (\H)\}$ scheduler,  we conjecture that $\bU_k \to $  a constant limit a.s.
 
 \noindent
{\bf Conjecture:}  For any SMR policy $d$  and any $\bbeta (\H,\bU)$ scheduler, we believe that 
$$
\bU_k (d) \to \rbU^*(d, \bbeta) \mbox{ a.s., }
$$ where $\rbU^*(d, \bbeta)$ is a constant a.s.  This conjecture can be proved either using  Law of Large Numbers for non-homogeneous Markov chains (\hspace{-.05mm}\cite{LLN}) or using stochastic approximation techniques (\hspace{-.05mm}\cite{Benveniste}). We are in the process of constructing this proof, for now we assume the conjecture to be true (see Fig. \ref{fig:conjecture}).

\begin{figure}[!h]
%\vspace{-4mm}
    \centering
    \includegraphics[trim = {2cm 0cm 0cm 0cm}, clip, scale = 0.3]{Figures/conjecture1.pdf}
    \caption{Convergence of average utilities to a constant}
    \label{fig:conjecture}
\end{figure}

By the above conjecture, 
under any SMR policy $d$ the $\bU_k$, converges to  a constant vector a.s., and hence the SMR policy will start depending only on the first component $\G_k$ of state vector $\X_k$,  and then $\{\H_k\}$ is close to a Markov chain; finally by Lemma \ref{lem_fixed_pt}, the algorithm used in   
\eqref{Eqn_beta_scheduler} converges to the optimal $\alpha$-fair objective function under that given SMR policy. 
Thus the Problem \eqref{Eqn_opt_original}  is equivalent\footnote{All the statements in this paragraph require proofs, we assume these and proceed further to derive online algorithm, which is the aim of this short paper.} to the following, where   the smaller domain $D^2$ includes SMR policies that depend only upon $\G_k$:
\begin{eqnarray}
 \label{Eqn_opt_reduced}
  \sup_{d \in {\cal D}^2} \sum_{n=1}^N \sbU^n_\infty (\bbeta^*) && \hspace{-7
  mm}\mbox{ where }
  \bbeta^* \in 
  \arg \max_{ \bbeta} \sum_{n=1}^N  \Gamma_\alpha \left ( \sbU^n_\infty \right )  \mbox{ with } \nonumber
\\
&&
\hspace{-23mm} \sbU^n_\infty \ := \
 \lim_{T \to \infty} \frac{1}{T}\sum_{k=1}^T   \sH_k^n \beta_k^n \
 \stackrel{a}=  \ E_{\rX_0}^d \left [ \sH^n \beta^n \right ].
\end{eqnarray}
Under any $d \in {\cal D}^2$,  $\{\G_k\}$ itself is a Markov chain,  with finite state space ${\cal S} =  \{ (1, \rsG) \mbox{ or } (\rsG, 1) : 1 < \rsG \le {\bar g}    \}.$ Hence    stationary distribution(s) exist and \underline{hence equality $a$ in} the above; when stationary distribution is unique, the stationary expectation $E^d[.]$ does not depend upon initial condition $\rX_0$. 

By Lemma \ref{lem_fixed_pt}, the inner optimization problem in \eqref{Eqn_opt_reduced} is solved for any $d \in {\cal D}^2$, the solution is given by \eqref{Eqn_beta_alpha_FP} and hence the problem further simplifies, for any initial $\rX_0$, to: 
\begin{eqnarray}
\label{Eqn_P3}
\sup_{d \in {\cal D}^2} \sum_n    \rsbU^n(d)  \hspace{-10mm}&& \mbox{ such that  for each } n, \\
\rsbU^n (d) &=& E^d_{\rX_0} \left[\sH^n  \Pi_{i \ne n}  \ind { \left \{ \frac{\sH^n}{ \left (\rsbU^n (d) \right )^\alpha }     \ge  \frac{\sH^i}{ \left (\rsbU^i (d) \right )^\alpha } \right \}  } \right ]. \nonumber 
\end{eqnarray}
Once again by Lemma \ref{lem_fixed_pt} and Law of Large Numbers for Markov chains (e.g., \cite{LLN}), one can re-write the above as the following average cost MDP problem,

\vspace{-3mm}
{\small \begin{eqnarray}
\label{Eqn_P3_avg}
\sup_{d \in {\cal D}^2} \lim_{T \to \infty} \frac{1}{T}\sum_{k=1}^T E\left [ \sum_n   \sH_{k+1}^n  \Pi_{i \ne n}  \ind { \left \{ \frac{\sH_{k+1}^n}{ \left (\sbU^n_k  \right )^\alpha }     \ge  \frac{\sH_{k+1}^i}{ \left (\sbU^i_k  \right )^\alpha } \right \}  } \right ],
\end{eqnarray}}
where $\{\bU_k\}$
are updated as in \eqref{Eqn_beta_scheduler}.
\begin{algorithm}[ht]
\caption{DOFS-initial condition $\rX_0$, $\epsilon$, $\alpha$, $\eta$, $\gamma$}
\label{algo_DOFS}
\begin{enumerate}
\item Initialize  $\bU_0$  and $Q(\rX,a)$ for all $\rX,a$ and set $k=0$, $\X_0 = \rX_0$.
\item  {\bf $\epsilon$-greedy age-scheduler:} With probability $\epsilon$,
  random (uniform) age-decision ($d$) is chosen, else  choose $d \in \arg \max_{a \in \{1, \cdots, N\}}Q(\X_k,a)$ .
\item Update age of all users, according to the following
\begin{eqnarray*}
&& \sG^n_{k+1} \leftarrow \min \left(\sG^n_{k}+1, \bar{g} \right ) \text{ if } n \ne d \text{ and,}\\
&& \sG^n_{k+1} \leftarrow 1 \text{ for } n = d.
\end{eqnarray*}
\item {\bf Data schedule:} For each $n=1,2,\cdots,N$, set
$$
\beta^n_{k+1}  = \prod_{i \ne n} \ind \left \{ \frac{\sH^n_{k+1}}{(\sbU^n_{k})^\alpha} \geq \frac{\sH^i_{k+1}}{(\sbU^i_{k})^\alpha} \right \}.
$$
\item Update average utilities, for each  $n$,
$$
\sbU^n_{k+1} = \sbU^n_{k}+\frac{1}{k+1}\left(\sH^n_{k+1}\beta^n_{k+1} - \sbU^n_{k} \right).
$$
\item Update \textit{Q-table entry} corresponding to $(\X_k, d)$, using {\small$\X_{k+1} = (\G_{k+1}, \bU_{k+1})$}:

\vspace{-5mm}
{\small 
\begin{eqnarray*}
\hspace{-5mm}
Q(\X_k,d) \ \leftarrow \ Q(\X_k,d) + \eta\bigg (\sum_{n=1}^N \sH^n_{k+1}\beta^n_{k+1} +\gamma \max_a Q(\X_{k+1},a)-Q(\X_k,d)\bigg )
\end{eqnarray*}}
\item Check some convergence criteria for $\bU_k$,
\begin{enumerate}
    \item If converged, then stop
    \item Else set $k \leftarrow k+1$ and go to Step 2
\end{enumerate}
%\end{enumerate}
%\item For $j=1,\dots,m$,
%  $$\bar{u}^\alpha_{j}\leftarrow\bar{u}^\alpha_{j}+ \frac{1}{t+1}\left(\u_j(\beta) - \bar{u}^\alpha_{j} \right),$$
\end{enumerate}
\end{algorithm}

\subsection{Online Algorithm-DOFS }

As mentioned before, we have an average cost MDP \eqref{Eqn_P3_avg}. From \cite{AvgtoDiscount},    the optimal policy for average cost MDP can be derived from that of the discounted cost MDP, when discount factor $\gamma$ is close to $1$. By this  observation, we propose an online algorithm which is based on two iterative algorithms: a) the well-known Q-learning algorithm  (e.g., \cite{RL}), and b) the iterative algorithm  that implements \eqref{Eqn_beta_alpha_FP} as in \cite{kushner,cellular}. 

In each time slot, first an age-decision is made using $\epsilon$-greedy scheduler, % (\hspace{-.05mm}\cite{RL}), 
which depends upon the Q-table estimates (as explained in Algorithm \ref{algo_DOFS}). Then an user for  data transfer is chosen using $\bU_k$ and $\H_{k+1}$; the latter are estimated (accurately)  after the user-position updates are obtained. 
Finally all the variables $\bU_{k+1}, \G_{k+1}$ and $Q$-table are  updated. 



\ignore{
\newpage 
\begin{eqnarray}
 \label{Eqn_opt_without_beta}
  \sup_{d \in {\cal D}^2}  \sum_{n=1}^N \Gamma_\alpha \left ( \bU^n_\infty \right ) \mbox{ where } \hspace{-20mm}
\\
\bU^n_\infty& :=&
 \limsup_{T \to \infty} \frac{1}{T}\sum_{k=1}^T   \H_k^n \beta_k^n \\
\beta^n_{k+1} &=& \Pi_{i \ne n}  \ind { \left \{ \frac{\sH^n_k}{ \left (\sbU^n_k \right )^\alpha }     \ge  \frac{\sH^i_k}{ \left (\sbU^i_k \right )^\alpha } \right \}  }
 \nonumber
\end{eqnarray}



we get optimal by solving the problem P.3  defined in \eqref{Eqn_P3}.


This is an average cost MDP problem. To derive an a more easy to solvable online algorithm (\cite{AvgToDiscount})
we model this problem as an infinite horizon discounted cost MDP with $\lambda \approx 1$:





%We assume that the user position updates can be obtained accurately. At the beginning of each time slot, the user's position information is updated. The BS then aligns the beams in the direction of the users and collect channel estimates for each of them. Based on the channel estimates and the average utility obtained by users so far, the data channels are allocated to one of the users according to $\alpha$-fair scheduler. We also assume that only one user can be served at a time.  Our aim in this work is to study the optimal policy which maximizes the sum utility of all the users.



\vspace{4mm}





%Any SMR policy $d$ makes user-position-update schedule decision based on $\X_k$  and then the channel gains are estimated in the aligned beam direction (according to the latest user-position updates).   Then opportunistic fair scheduler makes a data allocation decision for that slot. Then the average utilities so-far are updated as below:
%\begin{eqnarray}
%\sbU^n_{k+1} &=& \sbU^n_k + \frac{1}{k+1} \left ( \sH^n_{k+1} \beta^n_{k+1} - \sbU^n_k \right )  \nonumber \\
%\beta^n_{k+1} &=& \Pi_{i \ne n}  \ind { \left \{ \frac{\sH^n_k}{ \left (\sbU^n_k \right )^\alpha }     \ge  \frac{\sH^i_k}{ \left (\sbU^i_k \right )^\alpha } \right \}  }  \label{Eqn_beta_scheduler}
%\end{eqnarray}
%where $\sH^n_k = \sA^n_k \sU^n_k$, where  the amplitude  $\sA^n_k$ depends upon the age of that user-position update and  $\{\sU^n_k\}_{k}$ are IID across time-slots for any given user $n$. Thus, the optimization problem is,









%In view of this, we define the following optimization problems
\begin{eqnarray}
%\label{Eqn_P3}
\mbox{Problem: {\bf P}$_3$}
\nonumber \\
\sup_d \sum_n  \rbU^n(d) && \mbox{ such that } \\
\rbU^n (d) &=& \phi^n (\rbU (d), d) \mbox{ for each } n.\nonumber \hspace{20mm}
\end{eqnarray}
I can rewrite the above problem as:

%Multiply defined labels
\begin{eqnarray}
\label{Eqn_P3_mult}
\mbox{Problem: {\bf P}$_3$}
\nonumber \\
\sup_d \sum_n  \phi^n (\rbU (d), d) && \mbox{ such that } \\
\rbU^n (d) &=& \phi^n (\rbU (d), d) \mbox{ for each } n.\nonumber \hspace{20mm}
\end{eqnarray}

If $d^*$ is the solution then \begin{eqnarray}
\sum_{n=1}^N \rsbU^{n}(d^*) = \sup_d \sum_n  \phi^n (\rbU (d), d) \mbox{ such that } \\
\sum_{n=1}^N \rsbU^{n}(d^*) > \sum_{n=1}^N \rsbU^{n}(d) \mbox{ for all } d \text{ which satisfies } \eqref{Eqn_P3_?}
\end{eqnarray}

So is it equivalent to the following(?)
\begin{eqnarray}
\label{Eqn_Opt_problem}
\mbox{Problem: {\bf P}$_2$, find $\rbU^*$ such that the FP is solved} \hspace{-54mm}
  \nonumber \\
\sum_{n=1}^N \rsbU^{n*} & = & \sup_{d \in D^2}  \sum_{n=1}^N \phi^n(\rbU^*,d) \text{ where,} \\
\phi^n(\rbU,d) & := & \lim_{T \to \infty} \frac{1}{T} ..    \nonumber
\\
&\stackrel{a}{=}&\mathds{E}^d\left[\sH^n \Pi_{i \ne n}  \ind  \left \{ \frac{\sH^n}{ \left (\rsbU^n \right )^\alpha }     \ge  \frac{\sH^i}{ \left (\rsbU^i \right )^\alpha } \right \} \right], \label{Eqn_SD_util}
\end{eqnarray}
$E^d$ is stationary expectation generated under SMR policy $d=d^\infty$, 
and the optimization domain $D^2$ includes all the SMR policies which depends only on the age of position updates of each of the users. Observe that $D^2 \subset D^1$. Observe that $\A^n$ is a finite state-space markov chain under any SMR policy $d \in D^2$ and hence the existence of stationary distribution is guaranteed and hence the equality $a$. in 
}

\section{Non-opportunistic data scheduler}
\label{sec_noops}
In \cite{mmwave}, the authors consider  an optimal user scheduling problem to minimize the beam alignment overhead in mmWave networks, while maintaining the desired QoS (rewards related to data transmission) of each user. In each time slot, the BS selects one user, based on the information related to previous schedules and the beam search algorithm finds the most appropriate beam towards the selected user.
The time spent in aligning the beam, depends upon the  gap between the consecutive slots in which the same user is chosen.
As their purpose is different (maintain QoS, rather than maximize sum utilities as in  Section \ref{sec_model_Wireless}),  they do not collect channel estimates from all users in any slot.  Thus   their scheduler is non-opportunistic, as  opposed to the one  discussed in Section \ref{sec_model_Wireless}.  Further more, they do not consider fairness.


We propose two ways of introducing fairness into such schedulers and compare the same with DOFS in Section \ref{sec_examples}. 

\noindent {\bf Dual Non-opportunistic Fair Scheduler (DNOFS):} In each time slot, the scheduler uses the expected conditional channel estimates of the users $\{E[\sH^n_{k+1}|\G_k]\}$  in place of $\{\sH^n_{k+1}\}$,   for data-decision (in \eqref{Eqn_P3_avg}); here we assume $\sH^n_k = L^n_k\sU^n_k$, where $\sU^n_k$ are as before and  the factor $L^n_k$ depends on the age $\sG^n_k$ of user $n$ and   characterises the time lost in aligning the beam (using position update) to the user. The age-scheduler  depends only upon $\G_k$ as in previous section. DNOFS is presented in Algorithm \ref{algo_DNOFS}, which differs from 
Algorithm \ref{algo_DOFS} only in step (4).

\noindent 
{\bf Single Non-opportunistic Fair Scheduler (SNOFS):}
We now consider single decision in each time-slot as in \cite{mmwave}, and include the average utilities so far, $\bU_k$, directly in the objective function to achieve fairness, i.e.,  the age-MDP directly optimizes
the following:

\vspace{-4mm}
\begin{eqnarray}
\label{Eqn_M-DNOFS}
\sup_{d \in {\cal D}^2} \lim_{T \to \infty} \frac{1}{T}\sum_{k=1}^T E\left [ \sum_n  \frac{ L^n_{k+1}(\sG^n_{k+1}) \sU^n_k }{\left (\sbU^n_k  \right )^\alpha} \ind{_{\{n= d(\G_{k+1})\}}}   \right ]
\end{eqnarray}
Basically, the data and age scheduler coincide here.



 

 

 
\begin{algorithm}[!ht]
\caption{DNOFS-initial condition $\rX_0$, $\epsilon$, $\alpha$, $\eta$, $\gamma$}
\label{algo_DNOFS}
Steps (1)-(3) are as in Algorithm \ref{algo_DOFS}.
%\begin{enumerate}
 
%\item 

\hspace{.5cm} $(4)$ {\bf Data schedule:} For each $n=1,2,\cdots,N$, set
$$
\beta^n_{k+1}  = \prod_{i \ne n} \ind \left \{ \frac{E[\sH^n_{k+1}]}{(\sbU^n_k)^\alpha} \geq \frac{E[\sH^i_{k+1}]}{(\sbU^i_k)^\alpha} \right \}
$$

%\end{enumerate}
Steps (5)-(7) are as in Algorithm \ref{algo_DOFS}.
%\end{enumerate}
%\item For $j=1,\dots,m$,
%  $$\bar{u}^\alpha_{j}\leftarrow\bar{u}^\alpha_{j}+ \frac{1}{t+1}\left(\u_j(\beta) - \bar{u}^\alpha_{j} \right),$$
 
\end{algorithm}


 


\section{Numerical Experiments}
\label{sec_examples}

We perform exhaustive Monte Carlo simulations for the proposed DOFS, DNOFS and SNOFS algorithms under different mobility conditions: one where the users are static and other when the users are mobile. %The simulations are carried out for $N=2$.
We consider Rayleigh  channels and hence $\sU^n$ is exponentially distributed with parameter $\lambda^n$. We set $\lambda^1 = 1$, $\lambda^2 = 1.8$ and discount factor, $\gamma = 0.9$. We consider two users, i.e., $N=2$.

\noindent
\textbf{DOFS: } The factor $A_k^n$, which reflects the age dependent channel conditions, is considered to be a binomial random variable as below:
$$
A_k^n = 
\begin{cases}
\bar{a} & \text{with probability } p(\rsG^n_{k}), \\
\underline{a} & \text{else.}
\end{cases}
$$
For high speed users, the probability of good channel $p(\rsG)$ decreases fast with the age, $\rsG$. 
 For the purpose of simulations, we set $\bar{a} = 1.1$ and $\underline{a} = .3$. The values of $p(\rsG)$ can be seen from Fig. \ref{fig:static} and \ref{fig:mobile}. For example, $p(2)$ is 0.9 for static users indicating that the information is not deteriorating fast with time, while for mobile users $p(2) = 0.5$.
 In actuality, the users directly estimate $\sH_k = \sA_k\sU_k$
 when they measure their channels;
 also recall  the estimates are assumed to be accurate.

\noindent
\textbf{DNOFS: }As explained in Section \ref{sec_noops}, the BS  does not collect channel estimates from all the users, it instead utilises the conditional expected channel estimates, $E[\sH^n_k|\G_k]$ of the users as in Algorithm \ref{algo_DNOFS} and recall $\sH^n_k = L^n_k \sU^n_k$.  The factor ${ L^n_k}$ represents the loss owing to the time spent in beam alignment, which depends on the age of the previous position-information. We model it as in the following:
$$
E[L^n_k |\G_k=\rG]  = \frac{\bar{a}p(g^n) + \underline{a}(1-p(g^n))}{\bar{a}},
$$ so that   $E[L^n_k |\G_k] = E[A^n_k |\G_k]$; this is done to ensure fair comparisons. 

\noindent
\textbf{SNOFS: } Here the algorithm considers single scheduling decision, i.e., the same user is selected for   position-update and  data transfer in any time slot. To bring in  fairness, we consider the objective function as in \eqref{Eqn_M-DNOFS}.

%Check with $\beta^n_k = d$ and $\sH^n_k = \sH^n_k/(\bU^n_k)^\alpha$

\subsection*{Observations}
We analyse the case with $2$ users and observe the following (see Fig. \ref{fig:static} and \ref{fig:mobile}):
(i) The proposed dual scheduler, DOFS outperforms the existing schedulers, DNOFS and SNOFS, for all levels of fairness, $\alpha$; this fact is more clearly evident in the right side figures that have $\sbU^1_\infty+\sbU^2_\infty$ versus $\alpha$; (ii) as the fairness factor $\alpha$ increases, the utilities of the users close in, for all the three schedulers; thus the fair schedulers are effectively ensuring max-min fairness (that equalizes the utilities of all the users) as $\alpha \to \infty.$
 


\begin{figure}[!h]
\vspace{-12mm}
\begin{minipage}{7.5cm}
\centering
\includegraphics[trim = {0cm 0cm 0cm 1cm}, clip, scale = 0.35]{Figures/fig1 (1)_black.pdf}
%\includegraphics[trim = {0cm 0cm 0cm 1cm}, clip, scale = 0.18]{fig1.png}
%\caption{Utility of users under DOFS, DNOFS and SNOFS}
%\label{}
\end{minipage}\hspace{1.2mm}
\begin{minipage}{7.5cm}
%\vspace{-4mm}
\centering
\includegraphics[trim = {0cm 0cm 0cm 1cm}, clip, scale = 0.35]{Figures/sum_util_compare_static.pdf}
%\caption{ Sum utility of users under DOFS, DNOFS and SNOFS }
%\label{}
\end{minipage}
\vspace{-15mm}
\caption{ Utilities (left figure) and sum utilities (right figure) versus fairness parameter $\alpha$ for static users ($p(g) = [1, .9, .5, .1]$).}
\label{fig:static}
\end{figure}

\begin{figure}[!h]
\vspace{-16mm}
\begin{minipage}{7.5cm}
\centering
\includegraphics[trim = {0cm 0cm 0cm 1cm}, clip, scale = 0.35]{Figures/fig2 (1).pdf}
%\caption{Utility of users under DOFS, DNOFS and SNOFS}
%\label{}
\end{minipage}
\begin{minipage}{7.5cm}
%\vspace{-4mm}
\centering
\includegraphics[trim = {0cm 0cm 0cm 1cm}, clip, scale = 0.35]{Figures/1 plot second file (1).pdf}
%\caption{ Sum utility of users under DOFS, DNOFS and SNOFS }
%\label{}
\end{minipage}
\vspace{-17mm}
\caption{ Utilities (left figure) and sum utilities (right figure) versus fairness parameter $\alpha$ for mobile users ($p(g) = [1, .4, .2, .1]$)}
\label{fig:mobile}
\end{figure}

%\vspace{-3mm}
\section{Conclusions and Future Work}
The millimeter wave communications are the way forward towards supporting the high data-rate applications, as in 5G/6G networks. However, they pose serious design issues; the most complicated issue being the design of narrow and accurate beams directed towards each of the end-users. 

Opportunistic schedulers are known to provide  fair solutions, with a price of fairness that reduces as the number of wireless users increase (\hspace{-.5mm}\cite{mayur}).  Basically, the users with throughout `bad' channels  are allocated the slots when the opportunities  are the `best'  (possible as the channel conditions are independent across users as well as the time slot). 

The opportunistic schedulers require (accurate) estimates of channel conditions of all the users in all the time-slots. With millimeter wave communications that demand accurate beam alignment, one cannot derive channel estimates of all users in every time-slot. We instead propose to maintain a regular and sufficiently accurate estimates of user positions of all the users at the base station. Our inherent assumption is that the beam alignment is possible in negligible time with such accurate position-updates. We achieve this by optimizing the well-known alpha-fair objective functions that further depend upon the age of position-updates of various users.  

We finally propose an online-algorithm that simultaneously implements opportunistic-fair mmWave data-scheduler and an age-scheduler (that updates the user positions). We also propose two methods of incorporating (different levels of) fairness  into 
existing non-opportunistic mmWave-schedulers. We compare the performance of these schedulers with the proposed opportunistic schedulers; the initial simulation results show   that the latter significantly out-performs the former. 


This is just the beginning and we have several questions for future investigation. How will  the opportunistic schedulers fare with diverse users, some stationary and some mobile; which type of information (e.g., some estimates of user-speeds) enhances the design of such schedulers; how does the age-scheduler depend upon the statistics of the users; it might be more realistic to consider schedulers over finite-time horizons, how will the age-scheduler depend upon the time average utilities till that slot. 

==> symbols.tex <==
\chapter*{List of Symbols}
\label{ch:sym}
\addcontentsline{toc}{chapter}{\nameref{ch:sym}}
\makeatletter
%\newcommand{\tocfill}{\cleaders\hbox{$\m@th \mkern\@dotsep mu . \mkern\@dotsep mu$}\hfill}
\makeatother
%\newcommand{\abbrlabel}[1]{\makebox[3cm][l]{\textbf{#1}\ \tocfill}}
\newenvironment{symbols}{\begin{list}{}{\renewcommand{\makelabel}{\abbrlabel}
                                              \setlength{\itemsep}{0pt}}}{\end{list}}
\begin{symbols}
\item[$\mu$] 	Magnetic permeability
\item[$\mu_0$]	Magnetic permeability of free space
\item[$\varepsilon$] Relative complex dielectric constant
\item[$\varepsilon^{'}$]  Real part of dielectric constant 
\item[$\varepsilon^{''}$] Imaginary part of dielectric constant 
\item[$\varepsilon_{s}$] Snow surface dielectric constant
\item[$\varepsilon_{v}$] Snowpack volume dielectric constant
\item[$\kappa_e$] Volume extinction coefficient
\item[$\kappa_{a}$] Absorption coefficient
\item[$\kappa_{s}$]	Scattering coefficient
\item[$\delta_{p}$] Penetration depth
\item[$\delta R$]   Slant range resolution of SAR data
\item[$\delta R_g$]  Ground range resolution of SAR data
\item[$\mbox{c}$]	Speed of light
\item[$\lambda$]	Wavelength
\item[$\tau$] Pulse length of SAR signal
\item[$\beta$]  Bandwidth of the SAR signal
\item[$\theta$ ] 	Orientation angle 
\item[$\theta_{i}$] 	Incidence or local incidence angle
\item[$\theta_{r}$]  Local refractive angle 
\item[$\delta A$]	Azimuth resolution of the SAR data
\item[$L$]    SAR antenna length
\item[$\mathbf{E}(\mathbf{r},t)$] Electric field vector
\item[$\mathbf{E_{pq}^s}$]	Scattered field vector
\item[$\rho(\mathbf{r}, t)$] Volume density of free charges
\item[$\mathbf{g}_\mathbf{E}$] Stokes vector
\item[$g_0$] Total power of the wave
\item[$g_1$] Power in the linear horizontal or vertical polarized components
\item[$g_2$] Power in the linearly polarized components at tilt angles $\psi$= 45$^\circ$ or 135$^\circ$
\item[$g_3$] Power in the left-handed and right-handed circular polarized component
\item[$\mathbf{[J]}$]	Jones matrix
\item[$\bm{U_2}$] Unitary matrix ($\mbox{SU}_2$)
\item[$\lambda_1$, $\lambda_2$]	Non-negative real eigenvalues
\item[$A_W$] Wave anisotropy 
\item[$A_{p}$] Particle anisotropy
\item[$H_W$] Entropy
\item[$\mathbf{[S]}$]	$2\times2$ Sinclair matrix
\item[$\bm{k}$] 3-D Pauli target vector
\item[$\{\Psi_P\}$]	Pauli spin matrix set
\item[$\{\Psi_L\}$]	Lexicographic matrix basis set
\item[$\bm{\varOmega}$]	Lexicographic target vector
\item[$\mathbf{[T]}$]	$3\times3$ Coherency matrix
\item[$\mathbf{[C]}$]	$3\times3$ Covariance matrix
\item[$T^{*}$]	Matrix transpose with complex conjugation (superscript)
\item[$\langle ... \rangle$]	Spatial or temporal ensemble average
\item[$\sigma$$^\circ$]	Backscattering coefficient
\item[$\sigma_{hh}^0$]	Backscattering coefficient of $\mbox{HH}$ polarization
\item[$\sigma_{vv}^0$]	Backscattering coefficient of $\mbox{VV}$ polarization
\item[$\sigma_{vvhh}^0$]	Correlation coefficient between $\mbox{VV}$ and $\mbox{HH}$ polarization
\item[$\alpha_1$]	Dominant scattering magnitude
\item[$\mathbf{[T_2]}$]	$2\times2$ coherency matrix
\item[$m_{E}$]	Effective DOP
\item[$m_{E}^{\mbox{\scriptsize opt}}$]	Optimized AGU-Dop
\item[$p_{max}$]	Touzi optimum Dop (maximum)
\item[$p_{min}$]	Touzi optimum Dop (minimum)
\item[$\chi_{t}^{\mbox{\scriptsize opt}}$]	Optimum polarization angles (ellipticity)
\item[$\psi_{t}^{\mbox{\scriptsize opt}}$]	Optimum polarization angles (orientation)
\item[$s$]	RMS surface roughness
\end{symbols}

